Learning Multi-dimensional Human Preference for Text-to-Image Generation

Current metrics for text-to-image models typically rely on statistical metrics which inadequately represent the real preference of humans. Although recent work attempts to learn these preferences via human annotated images, they reduce the rich tapestry of human preference to a single overall score. However, the preference results vary when humans evaluate images with different aspects. Therefore, to learn the multi-dimensional human preferences, we propose the Multi-dimensional Preference Score (MPS), the first multi-dimensional preference scoring model for the evaluation of text-to-image models. The MPS introduces the preference condition module upon CLIP model to learn these diverse preferences. It is trained based on our Multi-dimensional Human Preference (MHP) Dataset, which comprises 918,315 human preference choices across four dimensions (i.e., aesthetics, semantic alignment, detail quality and overall assessment) on 607,541 images. The images are generated by a wide range of latest text-to-image models. The MPS outperforms existing scoring methods across 3 datasets in 4 dimensions, enabling it a promising metric for evaluating and improving text-to-image generation.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract_xxx.tex <==
\begin{abstract}

% Current evaluation for text-to-image models typically relies on statistical metrics which inadequately represent the real preference of humans. Although recent attempt to learn these preferences via human annotated generated images, they reduce the rich tapestry of human preference to a single overall score. However, when humans evaluate images across different dimensions (e.g. aesthetics, detail quality or semantic alignment), the regions of the image they focus on vary, which results in different preferences. Therefore, using a single score to encapsulate human preferences is insufficient. To this end, we introduce Multi-dimensional Human Preference Datasets (MHP), a large-scale dataset of generated images produced by a wide range of latest text-to-image models, which is annotated with human preferences from 4 dimension (i.e. aesthetics, detail quality or semantic alignment and overall assessment). The MHP comprises 918,315 human preference choices across 4 dimensions on 607,541 pairs of images. 
% Furthermore, we propose Multi-dimensional Preference Score (MPS) to learn these diverse preferences based on the MHP dataset. The MPS take the generated image, text and a certain dimensions of human preferences as inputs, and predicts a preference score for the current preference dimension.  
% Experimental results indicate that, compared to previous metrics, 
% our MPS achieves state-of-the-art performance in predicting human preferences across different dimensions and evaluating text-to-image models.
% Additionally, based on MHP dataset, we also establish a benchmark for evaluating recent text-to-image models.

We propose MPS, the first multi-dimensional text-to-image human preference reward model, to address multiple common concerns in current evaluations and align them with human values and preferences. Current metrics for text-to-image synthesis typically relies on statistical metrics which inadequately represent the real preference of humans, or inappropriately reduce the rich tapestry of human preference to a single overall score. However, the preference results vary when humans evaluate images with different aspects. To this end, we propose Multi-dimensional Preference Score (MPS), which introduce the condition module upon CLIP model to learn these diverse preferences.
% takes the prompt, generated image and a certain dimensions of human preferences as inputs, and predicts a preference score for the current preference dimension.
Its training is based on our Multi-dimensional Human Preference Dataset, which comprises 918,315 human preference choices across 4 dimensions (i.e., aesthetics, semantic alignment, detail quality and overall assessment) on 607,541 images. MPS outperforms existing scoring methods across 3 benchmarks and 4 dimensions, enabling it a promising metric for evaluating and improving text-to-image generation. The model and dataset will be made publicly available to facilitate future research. 




\end{abstract}

==> sec/4_method_xxx.tex <==
\begin{figure}[t]
\begin{centering}
\includegraphics[width=0.93\columnwidth]{img/framework.pdf}

\end{centering}
% \vspace{-4pt}
\caption{\label{fig:framework}
The framework of Multi-dimensional Preference Score (MPS).
The MPS takes the generated image, prompt and preference condition as the input, and predicts the quality (i.e. human preference) of the generated image under the given preference condition.
}
% \vspace{-8pt}
\end{figure}


\section{Multi-dimensional Preference Prediction}
% 先前的工作直接用clip来处理，对于多种偏好，虽然也可以用多个模型进行训练，但一旦改变偏好的条件时，就需要重新去学习，因而我们希望得到一个可以兼容不同偏好条件的预测模型。我们的方法是将某一种偏好设定成特定的单词（如），然后根据这些词去高亮出prompt侧的单词，然后在计算图片中的patch与这些prompt中的单词的相近时，只透过这些特定的token，以使得模型根据条件，取图像和文本中的不同区域进行预测，改变不同的条件只需要修改condition中的token即可
% Aesthetics: light, color, clarity
% Detail: shape, face, hands, structure
% Alignment: quantity, attributes, position, number
% Overall: light, color, clarity, shape, face, hands, structure, quantity, attributes, position, number
\subsection{Model Structure of MPS}

\noindent\textbf{Motivation}
Our motivation is computing the preference scores in difference preference conditions. 
Specific words in the prompt should be given more attention when given different conditions, e.g., when aesthetics is considered as a condition, words in the prompt related to color, light, and clarity should be taken into account more when calculating the score. Therefore, we propose a condition mask $M_c$ to highlight the relevant tokens while suppress the irrelevant tokens. 
The condition is represented by a series of attribute words, e.g. the preference condition of `Aesthetic' is represented by a set of words, including light, color and clarity. 

\noindent\textbf{Preliminary} As shown in Fig. \ref{fig:framework}, we adopt CLIP \cite{CLIP} to initially extract features from images and prompts. Given a prompt $x$ and an image $y$, the visual feature of $y$ is obtained by the vision encoder of the CLIP by $X_v=E_{v}(y)$, where $X_v \in \mathbb{R}^{n_v \times n_d}$. $n_v$ is the token number of the image and $n_d$ is the feature dimension. $X_t=E_{t}(x)$, where $X_t \in \mathbb{R}^{n_p \times n_d}$ and $n_p$ is the token number of the text. 

Previous work \cite{PickScore,HPS,ImageReward} typically utilize the first dimension of $X_v$ and the last dimension of $X_t$ to calculate the preference score, which loses a lot of detailed information of both image and text. Alternatively, we employ the full range of $X_v$ and $X_t$ and fuse two modalities through the Cross Attention (CA) module 
\begin{equation}
CA\left(X_{v},X_{t}\right)=\sigma\left(\frac{X_{v}W_{q}\left(X_{t}W_{k}\right)^{T}}{\sqrt{n_d}}\right)X_{t}W_{v}
\label{eq:cross}
\end{equation}
where $\sigma$ is the SoftMax activation function, and $W_* \in \mathbb{R}^{n_d \times n_d}$ are parameters and biases are omitted. 




\noindent\textbf{Preference Condition Module} The relevance of prompt and condition is computed by $R_{p,c}=X_{c}X_{p}^{T}W_c+b_c$, where $R_{p,c} \in \mathbb{R}^{n_c\times n_p}$, $n_c$ is the token number of the preference condition, and $W_c$ and $b_c$ are learnable parameters. The $R_{p,c}$ is averaged along the dimension $n_c$ and then repeated $n_v$ times to obtain the condition mask $M_c\in\mathbb{R}^{n_v\times n_p}$. 
The $M_c$ is further binarized to $\bar{M}_c$, where elements below the similarity threshold are assigned to negative infinity and others are set to zero.
Based on the condition mask $\bar{M}_c$, the Eq. \ref{eq:cross} is further improved as
\begin{equation}
CA\left(X_{v},X_{t}|X_c\right)=\sigma\left(\frac{X_{v}W_{q}\left(X_{t}W_{k}\right)^{T}}{\sqrt{d}}+\bar{M}_c\right)X_{t}W_{v}
\label{eq:cross condition}
\end{equation}
The Eq. \ref{eq:cross condition} ensures that the parts of the prompt that are  relevant to the condition information receive more attention when computing the preference score.
We adopt the first dimension (i.e. the cls token) of fused feature $CA\left(X_{v},X_{t}|X_c\right)$ for further prediction, which is denoted as $f_{v,t}$ and $s\in\mathbb{R}^{1\times n_d}$
Additionally, to prevent the issue of excessively short prompts leading to a scenario where no words of the prompt are related to the condition.
In such scenario, the cross attention layer would be unable to capture the information from the prompt. 
Therefore, we supplement the $f_{v,t}$ with additional prompt feature $f_t$, where $f_t$ is the last dimension of $X_t$. 
Consequently, the MPS is obtained by
\begin{equation}
S(x,y|c)=\alpha f_{v,t} \cdot f_t
\label{eq:MPS}
\end{equation}
where $\alpha$ is a learned scalar while $x$, $y$ and $c$ denote the prompt, image and preference condition, respectively.
% 为了防止prompt过短导致没有与condition相关的词语，在这种情况下CA将无法获取prompt的信息，为此我们在s的基础上额外再加入与原始的text信息，计算最终的得分为，s=，其中x为X_t的最后一维向量,is the learned temperature scalar

\subsection{Training}
The input for our objective includes our scoring function MPS $S(x,y|c)$, a prompt $x$, two generated image $y_1$, $y_2$, a preference condition $c$ and the preference score (annotated by human) $p$, where $p$ takes a value of $[1,0]$ for $y_1$ is preferred, $[0,1]$ if $y_2$ is preferred. 
Following previous work \cite{PickScore}, the training objective minimize the KL-divergence between the annotation $p$ and the softmax-normalized prediction
\begin{equation}
\begin{split}
&\hat{p}_{i,c}=\frac{expS\left(x,y_{i}|c\right)}{\sum_{i=1}^{2}expS\left(x,y_{i}|c\right)}\\
&L_{P} = \sum_{c}\sum_{i=1}^{2}p_{i,c}(log p_{i,c} - log \hat{p}_{i,c})
\end{split}
\end{equation}
We initialize the text and vision encoders, \( E_t \) and \( E_v \), with parameters from the pre-trained CLIP-H model, while the remaining parameters are subject to random initialization.
We train the our MPS on the training split of MHP datasets for 4,000 steps, with batch size of 128, with a learning rate of 3e-6, and with a warmup period of 500 steps.

